"Sharing, Not Showing Off": How BeReal Approaches Authentic Self-Presentation on Social Media Through Its Design

Adolescents are particularly vulnerable to the pressures created by social media, such as heightened self-consciousness and the need for extensive self-presentation. In this study, we investigate how BeReal, a social media platform designed to counter some of these pressures, influences adolescents' self-presentation behaviors. We interviewed 29 users aged 13-18 to understand their experiences with BeReal. We found that BeReal's design focuses on spontaneous sharing, including randomly timed daily notifications and reciprocal posting, discourages staged posts, encourages careful curation of the audience, and reduces pressure on self-presentation. The space created by BeReal offers benefits such as validating an unfiltered life and reframing social comparison, but its approach to self-presentation is sometimes perceived as limited or unappealing and, at times, even toxic. Drawing on this empirical data, we propose design guidelines for platforms that support authentic self-presentation while fostering reciprocity and expanding beyond spontaneous photo-sharing. These guidelines aim to enable users to portray themselves more comprehensively and accurately, ultimately supporting teens' developmental needs, particularly in building authentic relationships.

==> graveyard-discussion.tex <==
\section{Discussion}
Peer relationships play a crucial role in adolescent development, and reciprocal and authentic self-disclosure is necessary for these relationships to develop. Despite the significant role of social media in facilitating such adolescent peer interactions, its capacity to support authentic self-disclosure is often compromised, for example, by context collapse and the pressures of self-presentation. This study delves into BeReal, an app distinguished by its focus on fostering authentic exchanges, and its success in gaining popularity among adolescents.

Our research examines BeReal's development of an authenticity norm and assesses its alignment with the developmental and self-presentation needs of teens. Here, we (1) identify design elements that led to the successful cultivation of authenticity norms on social media, (2) analyze the developmental and individual needs of users that remain unfulfilled under the authenticity definition that BeReal prescribed, (3) introduce the Self-Disclosure Authenticity Matrix to guide the shaping of authenticity norms cognizant of teens' peer-relationship-building needs, and (4) propose design recommendations for authentic sharing on social media derived from the Self-Disclosure Authenticity Matrix and our study findings.


% \subsection{Evaluating the Prescriptive Design of BeReal}
% BeReal cultivates an authenticity norm of ``being real'' by sharing daily, unfiltered, in-the-moment photos through several design shifts that break from the common interface patterns found in other social media platforms. First, while most photo-centric platforms popular among adolescents permit content editing, BeReal discourages filters and encourages spontaneous photos. Second, BeReal takes pressure off the act of choosing to post by providing an air cover for frequent sharing via its daily notifications. Furthermore, interactions on mainstream platforms are heavily quantified through likes and comments. BeReal, conversely, makes these metrics ephemeral, disappearing with each post, thereby reducing the intensity of comparisons and taking pressure off posting. Third, many platforms monetize through scale, inadvertently promoting a proxy for social status through public network size quantification, leading to context collapse. BeReal, however, conceals friend counts and advocates for smaller network sizes, fostering safer, more communal spaces. Finally, BeReal's design is minimalistic and centered around the theme of authentic photo sharing, making it clear to the users what BeReal is meant to be for. These findings demonstrate that social media platforms can, through designs, create a strong sense of a platform norm among its users, strong enough that users engage with the platform in ways that were deemed not possible on any other social media platforms in general.

\subsection{BeReal and Authentic Self-Presentation}

self-presentation is innately social
- The real or anticipated reactions of other people to this information influence the timing, form, and content of self-presentational activity.
- Symbolic interactionists such as Mead (1934) and Cooley (1902) were among the first to emphasize that actions carry symbolic meanings that influence the responses of others to self.
- Goffman (1959) elaborated the theme when he described social life as a series of performances in which people project their identities or “faces” to others and engage in mutual activities that are governed by social rules and rituals.
- Self-presentation is also likely to involve controlled processes when the situation or audience is significant or the actor is uncertain about the type of impression that might be created (Schlenker, Britt, \& Pennington, 1996; Schlenker \& Pontari, 2000). Under these conditions, people focus, often self-consciously, on the impression they might make and try to plan and rehearse their performances. 
- Self-presentation reflects a transaction between self and audience in a particular social context (Schlenker, 1985; Schlenker \& Pontari, 2000). It is not purely an expression of self, purely a role-played response to situational pressures, or purely conformity to the identity expectations of salient others.

BeReal is trying to move away from inauthentic self-presentation to authentic, spontaneous self-presentation
- These characterizations attempt to distinguish between what might be called self-expression, which is viewed as authentic, spontaneous, and originates from within the actor, and self-presentation, which is portrayed as inauthentic, labored, and influenced by social pressures.
- the main way they do that is by carving out a safe space. Self-presentation scripts can be cued automatically by specific features of the audience and situation, and actors are often unaware of the extent to which their behavior is influenced by the social context and their own interpersonal goals In the realm of self-presentation, automaticity seems most likely to occur when people are in familiar situations with people they know well and in whose positive regard they feel secure (e.g., relaxing at home among friends).
- People generally are more self-enhancing with strangers and more modest with friends (Tice, Butler, Muraven, \& Stillwell, 1995). With friends, modesty is the more automatic style because people are relatively secure in their friends’ regard and need not brag. If people are induced to present themselves in a way that differs from the automatic style, it will require greater cognitive effort and interfere with the capacity to accomplish other cognitive tasks, such as remembering information about the interaction.
- trying to condition automaticity too

self-presentation on BeReal can be particularly difficult, esp. for some
- expression is limited and accurate self-presentation or use of tactics can be more difficult; It is a combination and reflection of all of these, incorporating features of the actor’s self-concept, personality style, social roles, and beliefs about the audience’s preferences. Even if people do not usually see themselves as having a specific set of attributes, they can readily imagine exemplars for how particular types of people should
- complemented by the 2 minute time limit (increase in cognitive load used as an advantage)
- Furthermore, it appears to take as much self-presentation skill to communicate an accurate, truthful impression as it does to convey a false one. (esp. given random notifications + limited medium)
- Self-presentation also should be more automatic when it involves qualities that are consistent with existing self-images and personality characteristics. (if not presentable - then 2 minute + not automatic for social media -> overwhelming)
- the worst case is when there is so much discrepancy that BeReal further encouraged some teens to ignore their internal cues
    - Many problems in social life arise from a single-minded focus on gaining approval and acceptance from immediate audiences. Outer orientations are associated with social trepidations.
    - Thus, attempts to look good to immediate audiences can increase health risk.
    - It is worth noting that these are not really self-presentation problems, they are outer orientation problems. They arise because people are focused on gaining the approval and acceptance of immediate others and will do whatever is necessary, including ignoring their own principles and good judgment, to impress others. Everyone cares about acceptance and approval.
    - Hogan and Cheek (1983) proposed that maturity involves being able to deal with both inner (e.g., personal principles) and outer (e.g., the expectations and preferences of others) concerns. To be oriented exclusively toward outer concerns is to allow others to dictate one’s life. Conversely, to be oriented exclusively toward inner concerns often amounts to being egocentric, eccentric, and unable to deal effectively with others. Balancing inner and outer concerns evidences more mature functioning.

self-presentation is not necessarily bad
- Self-presentation is not just superficial, deceptive, or manipulative activity. It can also involve attempts to convey to audiences an “accurate” portrait of oneself 
- The objective may be to ensure that others view one appropriately (i.e., in ways that secure the desired regard and treatment associated with one’s identity), to receive validating feedback that might minimize personal doubts about what one is really like, or even to follow the principle that “honesty is the best policy” and thereby feel authentic while minimizing the hazards of deceit.
- Thus, although self-presentation involves the packaging of information in order to accomplish goals, the goals can include conveying an authentic portrayal of self (as the actor sees it), not just a deceptive one (Schlenker \& Pontari, 2000).
- Whether low-self-monitor or high, everyone has motives for self-presentation; low self-monitors are concerned about their “reputations of being genuine and sincere people who act on their beliefs.”
- and so being truly "authentic" may be unachievable, whatever that means; it's especially difficult to expect the level of maturity to balance outward and inward facing motivations in teens

BeReal is trying to push toward a part that's more conducive to intentional 
platforms can support intentional or automatic, and both directions can be authentic but push notification is by definition making things intentional rather than automatic; which is contradicting with intentional 
user is initiating the push button to share both front and back unfiltered, and that's pretending to be automatic rather than intentional; people are being authentic-intentional but BeReal is pushing toward automatic-authentic
automatic = doing without knowing; so push notification by definition is not automatic

% Our findings reveal ways in which BeReal's current design substantially fails to meet adolescents' developmental and self-presentation needs for authentic interpersonal sharing. While all participants appreciated BeReal's effots to encourage more authentic sharing on social media and many felt that BeReal successfully did so at the community-norm level, participants were not as satisfied with BeReal's norms as individual users. Here, we present three shortcomings of the prescriptive design of BeReal.

% \vspace{2mm}
% \noindent\textbf{Fragmentary.} A critical challenge with BeReal's approach to authenticity is its narrow definition, which does not accommodate varied personal interpretations of what being ``authentic'' entails. This rigidity led to dissatisfaction among users who view authenticity through a broader lens. They saw other interpretations of authenticity that BeReal did not support, such as sharing their deeper identities and thoughts. Some even felt that curating---what is considered inauthentic under BeReal's authenticity definition---is part of efforts to be authentic: feeling uncomfortable about what one shares makes what they share inauthentic immediately, and so by curating they feel comfortable with what they share. For these users, curating means that others are presented with what they actually care about, rather than random moments the platform told them to share that do not hold much personal significance to those sharing. This suggest a disconnect between BeReal's idea of authenticity and the nuanced ways teen users individually perceive and practice authenticity.

% \vspace{2mm}
% \noindent\textbf{Unconvincing.} BeReal's definition of authenticity was seen as unattractive to some users. The app's straightforwardness, while preventing users from becoming overly absorbed, also led to an experience some described as underwhelming. Many users said that they thought of or saw other users ending up leaving the app because it has an underwhelming user experience. Users expressed concerns about the repetitiveness and mundanity of posts, both their own and others', fearing judgment from friends for being perceived as uninteresting. This apprehension prompted a few to stage their posts or disengage from the app altogether. Despite appreciating the concept of showcasing unfiltered life, the daily portrayal of ordinary life lacked appeal for many.

% For a portion of the user base, the concept of achieving true authenticity on social media was met with skepticism. While the initiative behind BeReal was appreciated, some users doubted the feasibility of fostering genuine authenticity within the inherent self-presentational dynamics of social media platforms. This skepticism was compounded by the belief that the responsibility for fostering authenticity lies beyond the app's capabilities, framing BeReal as a platform for entertainment or memory-keeping rather than a transformative social media experience.

% The divergence in users between those who embraced the platform's norms and those who did not, underscored a challenge in maintaining a collective adherence to the authenticity norm on BeReal. Because a significant part of the norm is reciprocity, the norm of the platform being intact depends a lot on the collective effort of all users to uphold the norm. However, when a subset of friend circles started to \textit{``cheat''}---either by (allegedly) staging or posting blank photos to view others' without actually sharing---led other people in the circle feel demotivated to be authentic. Because being authentic on social media where people usually share their well-put-together selves required a degree of vulnerability, that vulnerability being one-sided (not reciprocated) led users to feel disappointed and like their mutual trust has been broken, which contrasts with the \textit{``communal''} feeling that BeReal gives when users perceive like they are participating, with their trusted friends, in part of a larger effort to make social media better.

% \vspace{2mm}
% \noindent\textbf{Backfiring.} BeReal's persuasive elements encourage adolescents to ignore their own internal cues about whether to disclose or withhold, at times pressuring them to share when they would prefer not to. Some simply felt uncomfortable and/or vulnerable sharing their unfiltered and uncurated selves, and felt that social comparison may be exacerbated on BeReal, for example, when they feel like their curated selves are not as glowy as others' uncurated selves. And yet, because they have to post in order to see others' posts, they ended up sharing in moments when they felt like they did not want to out of fear of missing out. However, other users whose thoughts and/or needs aligned with BeReal's and saw BeReal's features as conveying definitions rather than interpretations, led efforts to reinforce the norms of BeReal by policing other users that were failing to be sufficiently ``authentic'' and breaking the norms of the platform. This often incited new forms of toxicity, for example, where the users would compare against each other in terms of how ``authentic'' they are, by comparing the number of retakes.

% In fact, the constant awareness of what is going on with peers' lives gave some of them extra insecurities that their own lives are not as interesting enough or that they are being excluded from their friend groups. While some participants shared that they felt good about getting the behind the scenes lives of peers that are \textit{``always looking fabulous I'm always feeling fabulous and nothings wrong in my life''} (P02) that reminded them that everyone is human. However, regardless of whether they were staged or not, BeReal posts often reminded users of how less interesting their lives seem to be in comparison to those of \textit{``the more popular kids''} (P28).


\subsection{Authenticity and Relationship-building on Social Media}
\input{tables/diagram}

\vspace{2mm}
\noindent\textbf{The Self-Disclosure Authenticity Matrix.}

According to the Social Penetration Theory (SPT) \cite{carpenter2015social}, healthy adolescent relationship-building requires gradual increases in intimacy and a precision approach to self-disclosure in a reciprocal manner \cite{berger_social_2015}. As dyads reciprocally exchange information about themselves, their breadth and depth of self-disclosure increases. To anchor our discussion of whether self-disclosure and authenticity are supported in such a way on BeReal, we illustrate the SPT in a matrix as shown in Figure \ref{fig:diagram}. The \textit{casual-intimate} axis captures the depth of user self-disclosure, ranging from everyday details (casual) to deeply personal ones (intimate). The \textit{limited-robust} axis captures the breadth of user self-disclosure, ranging from a narrowly defined slice of a user's life (specific) to all facets of it (comprehensive). Combining these two axes creates a matrix describing four types of authentic self-disclosure that sociotechnical spaces for relationship-building should be able to support. Central to all such authentic self-disclosure is the norm of reciprocity. Here, we describe these four categories and provide examples for each.

\begin{itemize}
    \item \textbf{Casual-specific authenticity.} In social media platforms that adhere to a casual-specific authenticity norm, users are encouraged to disclose lighthearted, casual details about a narrow segment of themselves. The culture on BeReal, for the most part, exemplifies this type of authenticity norm, with users encouraged to share photos of ordinary moments and to share only about their daily lives (rather than their opinions, identity, personality, or preferences).

    \item \textbf{Casual-comprehensive authenticity.} On platforms that foster casual-comprehensive authenticity norms, users are encouraged to share any content about themselves that is lighthearted and less revealing. Participants cited Finsta accounts and Close Friends Stories as examples of such social media spaces.
    
    \item \textbf{Intimate-specific authenticity.} Platforms characterized by intimate-specific authenticity norms typically encourage intimate user disclosures within a defined scope. Previous research \cite{Barta2021-yh} studying TikTok users' experiences creating and consuming content illustrates a particular case of social media usage that exemplifies this dynamic. The study describes how, despite TikTok's design enabling intimate self-disclosure in general through affordances such as anonymity, viewers have very little context about anonymous creators' larger lives and impose high standards of narrative consistency. Specifically, the study mentions the audience judging creators' authenticity based on their perceptions of the creators, informed by the creators' past activities and content. Consequently, self-disclosure beyond certain topics of interest or identities becomes rarer.
    
    \item \textbf{Intimate-comprehensive authenticity.} Platforms exhibiting intimate-comprehensive authenticity norms facilitate all varieties of disclosure. One-on-one communication spaces such as Snapchat's private story and Discord's direct messaging with the innermost circle of friends exemplify this.
\end{itemize}

\vspace{2mm}
\noindent\textbf{BeReal and the Self-disclosure Authenticity Matrix.}
BeReal is a relationship-forward platform in which the interactions can be evaluated using the matrix. The fundamental idea behind BeReal promoting \textit{``authentic''} photo sharing, according to BeReal, is to connect with \textit{``your friends for real''} \cite{noauthor_undated-pl} and to make \textit{``meaningful connections''} by sharing a \textit{``genuine glimpse''} into users \textit{``real life''} with the people that users \textit{``care most about.''} A relationship-forward social media should ideally support interactions from the \textit{casual-specific authenticity} quadrant to the \textit{intimate-comprehensive} authenticity. Relationships at different stages require different types of authenticity across the four quadrants.

However, not all participants found the platform effective in building relationships. On BeReal, users communicate in one way: sharing in-the-moment photos of themselves. Though users may be able to express themselves deeper and with more breadth in some cases, such as long-distance friendships, they found interactions on BeReal to be limiting and restricting. Several participants shared desires to share more diversified aspects of themselves, such as their performances, or to express more intimate aspects of themselves, such as thoughts, through text. While users can add captions and comments to the photos, as the posts are not accessible after a day, leaving comments became less of a norm, leading users to feel like they cannot communicate much on BeReal.

Another issue on BeReal related to social penetration is that the reciprocity norm often failed because sharing unfiltered, unstaged photos of themselves was perceived to be at different levels of breadth and depth for each user. For some, sharing unfiltered photos was not of concern, and they had many ``interesting'' things going on in their lives that they could share with their friends even while being ``authentic.'' In such cases, sharing BeReal posts was mostly perceived as being casual and low pressure. However, for others, sharing their unfiltered lives was high-pressure and something that they could only share with their closer, more intimate friends when their BeReal friends also consisted of friends they are not very close with. The latter group of users consequently felt more uncomfortable posting on BeReal, leading them to disengage or ``cheat.'' Reciprocation then failed.

\subsection{Design Recommendations for Online Authenticity}
Guided by the Self-disclosure Authenticity Matrix and informed by data derived from our study, we propose design recommendations for fostering online authenticity.

\begin{itemize}
    \item \textbf{Scaffold reciprocal disclosure.} According to the SPT, mutual disclosure is an essential component of the progression of social penetration. However, many mainstream social media platforms such as TikTok which primarily follow a one-to-many disclosure pattern, often fail to facilitate social penetration despite extensive user engagement. To normalize reciprocity and foster social penetration at an individual or community level, designers might consider introducing covers to minimize the vulnerability associated with initiating online engagement. As reported by our participants, daily post notifications relieved the pressure of sharing on social media, fostering a sense of community and a collective effort toward online authenticity. Thus, strategies such as daily reflection prompts might serve to diminish the vulnerability associated with initiating disclosures and encourage more users to reciprocate in intimate self-disclosure contexts.

    \item \textbf{Support different stages of relationships.} While BeReal focused on promoting authenticity primarily in a casual and scoped sense, there exist other forms of authenticity, as illustrated by the Self-disclosure Authenticity Matrix. Platform designers may consider the implications of the matrix to create social media spaces that support relationships beyond a single quadrant. For example, if a platform aims to serve beyond casual-specific authenticity, offering means of expression beyond photos could support more intimate self-disclosure. While options such as text or live photos may not guarantee more intimate sharing, they could serve as foundational prerequisites. Our study results also suggest that a smaller and more closely knit audience might foster comprehensive disclosure. Given that some of our participants expressed difficulty in rejecting friend requests, design mechanisms might offer users a convenient `excuse' or safeguard to actively curate their audience. \footnote{While our example discussed design directions toward higher levels of self-disclosure, the discussion of supporting users with more intimate and comprehensive authentic self-disclosure is meant to address the difficulty of achieving such levels rather than suggest their inherent superiority. No single form of authenticity is universally preferable. As per the SPT, different authenticity types simply cater to relationships at different stages. For example, while 1:1 messaging can support all forms of authenticity, it might be deemed too intimate and cause discomfort when used with casual acquaintances.}

    \item\textbf{Prevent Weaponized Authenticity.} Participants said that authenticity norms turned toxic when the platform pressured them to over-disclose or enabled users to shame one another, police one another, or compete to be the most authentic. Through intentional design decisions, platforms can encourage candid sharing without making an idol of it. For example, a platform might avoid quantifying authenticity by choosing \textit{not} to display the number of times a photo was retaken.

    \item\textbf{Scafford users toward platform norms.} For platforms prescribing the ideal behaviors and norms, it is crucial to convince as many users as possible to onboard with the platform's norms to ensure long-term success. As observed on BeReal, when a subset of users disagrees with the norm, the collective effort to follow the norm can collapse due to the break of reciprocated trust. However, it is inevitable that all users will have different stances and experiences with platform designs and norms. Therefore, rather than enforcing prescriptive norms on all users, meeting individual users where they are and scaffolding them toward what the platform ultimately aims could be a good approach.

    \indent For BeReal, users who are more shy could start off at different levels of self-disclosure, where the lowest level could be users receiving a daily prompt to share how they are feeling or what they are doing, but only in text form; then in next level, instead of daily random notifications, users get weekly prompts for photos related to specific, broad themes (e.g., ``parts of my room,'' ``Something Blue''). This gives users more time to consider their submission and aligns with a broader theme, reducing the pressure of capturing a spontaneous moment. In the third level, similar to BeReal's concept but with an option to skip the prompt or extend the time limit. Users can also select \textit{``comfort zones''} that limit when and where notifications for photos are received, such as only during certain hours or in certain locations.

    \item\textbf{Provide air cover for casual, low-effort sharing.} On mainstream social media platforms, users are presented with many different features that they can choose to engage with. In other words, users bear the burden of making active decisions about what, when, and how to share. This responsibility can be daunting, as every post made on social media becomes a reflective mirror, often leading to increased pressure and anxiety. BeReal, in contrast, provides stricter user guidelines, mitigating much of this decision-making pressure. As a result, BeReal users collectively were comfortable enough to share more raw, and often consequently more vulnerable, photos with their closer group of friends despite the cultures on other social media platforms that they are used to that promote otherwise.
\end{itemize}

It is important to note that while self-disclosure is generally desirable for social penetration, pursuing it online could introduce potential risks or unforeseen consequences not typically present in offline settings. Younger users, especially those with problematic smartphone use \cite{Davis2023-zk} are even more likely to disclose beyond what may deemed the appropriate level of self-disclosure. Therefore, when designing to expand the breadth, depth, or frequency of online self-disclosure, it is essential to anticipate potential harmful outcomes to users, such as online harassment or impersonation. Designers should rigorously test their designs with a diverse user group to ensure no targeted group faces heightened risk, implement robust privacy and security measures on the platforms (e.g., disabling screenshots), and possibly guide users to understand and reflect on their desired level of self-disclosure and/or social penetration online.


\subsection{Limitations and Future Work}
Our study has several limitations. The first is that our participant sample includes significantly more people identifying as girls than as boys or non-binary. Further, BeReal introduced many new features since our data collection: (1) the integration of Spotify, where the cover art of the song or podcast a BeReal user is listening to will appear in the bottom right corner of their post, (2) a bonus BeReal where BeReal allows users to post an additional two BeReals throughout the day — but only if they post their first during the allotted two-minute window, (3) branded accounts (e.g., Adidas, Notion), and (4) ``Groups'' which resemble group chats to name a few. A lot of how the platform norm is perceived is likely would have changed with the introduction of the new features. It would be useful for future work to explore how this extra disclosure and extra element of gamification support or undermine healthy and desired forms of authenticity or create further privacy concerns or pressure.

Future studies might also consider exploring methods to support more comprehensive authentic sharing integral to adolescent relationship-building. Specifically, while BeReal's design indeed offers a new approach to social media---encouraging users to share more authentically---our study's participants highlighted that the platform focuses primarily on one facet of authenticity: transparent photo sharing. They also mentioned the presence of potentially harmful, undesired, or incomplete forms of authenticity on BeReal. As a result, there remains a need for future research to explore novel designs that could foster and normalize different facets of authenticity that transcend a single form of authenticity on social media, moving towards, for example, more intimate or comprehensive authenticity that our participants expressed a desire for.
